Privacy or Transparency? Negotiated Smartphone Access as a Signifier of Trust in Romantic Relationships

In this work, we analyze two large-scale surveys to examine how individuals think about sharing smartphone access with romantic partners as a function of trust in relationships. We find that the majority of couples have access to each others' devices, but may have explicit or implicit boundaries on how this access is to be used. Investigating these boundaries and related social norms, we find that there is little consensus about the level of smartphone access (i.e., transparency), or lack thereof (i.e., privacy) that is desirable in romantic contexts. However, there is broad agreement that the level of access should be mutual and consensual. Most individuals understand trust to be the basis of their decisions about transparency and privacy. Furthermore, we find individuals have crossed these boundaries, violating their partners' privacy and betraying their trust. We examine how, when, why, and by whom these betrayals occur. We consider the ramifications of these boundary violations in the case of intimate partner violence. Finally, we provide recommendations for design changes to enable technological enforcement of boundaries currently enforced by trust, bringing access control in line with users' sharing preferences.

==> attitudes.tex <==
\section{Attitudes about Sharing}
\peri{there are a million numbers here but I think this section will benefit greatly from inclusion of strategic numbers and free text responses, as well as some of the 'why' questions from symantec. more than stating what people said and where there are demographic trends (which I will still do) I think the best point we can make is that it's messy, ambiguous, and there isn't consensus, not even consensus among similar people - it's all squishy and contextual and, well, human}

Access to someone's phone is fairly binary---you have it or you don't. However, this access allows you to do a lot of different things, some of which a partner may be comfortable with, and others which may be intrusive. In an effort to demonstrate that this is the case, we asked respondents about a series of behaviors, with respect to whether they were common and whether they were good. 

All respondents were asked these questions, regardless of their relationship status, as the goal was to establish a sense of a cultural norm about where the line is when accessing a partner's phone. In addition to the numerical data, we have free text responses from these sections which provide context to these answers, and demonstrate the nuance that can make these questions difficult to answer. Symantec's data also asked follow up questions of anyone who indicated they had taken particular actions, asking why they had done so, though this data is also multivariate.

\subsection{Everything is Relative}
There is little consensus about what is or is not normal or good. Perceptions vary widely by age and relationship status (again, intertwined) as well as by gender. Some of the comments provide clarity to this - a behavior which may be normal and desirable ten years into a marriage might be concerning six months into a relationship. 


\subsection{What the hell is trust}
It is clear that the expectations of access and use of access are predicated on trust in a relationship. What that looks like, however, is not widely agreed upon. Opposite behaviors were explained in almost identical language: "we don't need access - we trust each other!", "we have access to everything - we trust each other!"

Either one trusts their partner not to misbehave enough to refrain from accessing their phone, or one trusts their partner not to abuse access to their phone. There is a "nothing to hide nothing to fear" attitude here as well. While there is mention of causes for distrust that are \textit{not} infidelity, the preponderance of reasoning and justifications offered for snooping relate to cheating. This is reflected in Symantec's data as well. 
Notable mention of using a tracking app to ensure a recovering alcoholic was not at a bar, a few entries for checking search history for porn. One woman notes that "the weaker person in the relationship may feel safer if they are being tracked" so... it's complicated.

\subsection{consent is key}
Regardless of whether people felt that trust in the relationship was reflected through privacy or transparency, there was generally consensus that whatever access there was had to be consensual and mutual for it to be healthy. People understood that in having access to a partner's phone they inherently had the capacity to read their DMs, but that didn't make it ok to do so, unless that was something they had discussed. While it's great that people understand this, there were plenty of respondents who also indicated that they go through their partner's phone when they're asleep, and similar things, so it's clear that this trust is abused. Again, the case being made here is for access that is less all or nothing.

==> datasets.tex <==
\section{Datasets}
\label{sec:datasets}



\subsection{Our Data}

Participants were all adults living in the United States who used a smartphone on a daily basis. 
Those under 18, in other countries, or who did not use a smartphone were disqualified. 
Participants who were not in relationships were still invited to participate, though there were several sections they were not shown.
Participants were recruited both via Facebook advertising and through Prolific.
%Responses with answers for fewer than 75\% of the questions they were asked were excluded, as well as those with failed attention checks 

or completed in an unreasonably short amount of time were excluded from analysis. 
After this, we had a total of \peri{check this} 538 respondents. 
In Table \ref{tab:demo} we provide a demographic breakdown of our sample.



%\subsection{Other}
%Reserving space because there are plenty of other papers that have one or a handful of relevant stats that help make our point and I anticipate something of an SoK vibe emerging here in that we can say ok we have this large dataset and that's half the contribution and the other half is we wrangled one number from here and one number from there etc. 

==> misc.tex <==
old abstract

    There has been much research on the propensity of individual users to share their mobile devices and site credentials with those they care about, and about the consequences of the abuse of that trust. Little is understood about how society as a whole thinks about this device sharing. We perform the first empirical analysis of users' behavior, perceptions of others' behavior, and estimations of societal norms with respect to smartphone sharing, appropriate use of access, and credential sharing. We combine new data from a large-scale, in-depth survey with other data addressing specific pieces of this question to assemble an understanding of Americans' digital privacy and security postures with respect to their partners, what they perceive to be normative in this regard, and where users draw the line between positive sharing and negative intrusion. Finally, we include a partner violence screen to better identify which behaviors should - or should not - be concerning to advocates in this space.
    
old intro

\peri{this is mostly narrative for now and does not have the standard "in this paper we will..." -- I got on some tangents and intend to take much of this out and use it in the intro for the thesis instead but I'm leaving it here for now since you might have feedback -- it's a little all over the place and possible repetitive but I'm moving on instead of spending a long time editing an intro for a paper I haven't written}

Information and computer security as fields have long focused on threat models involving sophisticated external attacks on large scale, often corporate or governmental, systems. 
As such, much emphasis was put on constructing strong defenses at the perimeters of these systems, and less consideration was given to what happened within the fortressed network.

With the advent and proliferation of consumer technology, a similar model of security emerged: use strong passwords, don't share them, and hope for the best. 
If we think about a user's combined devices and accounts in the way we might think about a corporate network, it operates in this model -- access to one thing begets access to the rest. 
Even as two factor authentication has become more common to address the concern of stepping-stone access stemming from a breech of forgotten Yahoo and Hotmail accounts, 2FA is almost always reliant upon a particular device, again leaving the user's "network" with complete trust after one point of access. \cite{yourself from google about relative frequency of 2FA}

Over time, as systems grew and network connections abounded, it became clear that a strong external defense was insufficient in corporate and governmental contexts. It is hubris to assume an attacker will never penetrate defenses, and foolish to allow them free reign once they do. 
Further, there is a strong layer of \textit{human} trust involved in assuming that no authorized users will abuse their access.
"Zero Trust" is now considered a gold standard in the design of networked systems\footnote{It is so much so that there are fields (i.e. blockchains) where zero trust has become provable}: access control should be strictly limited, authentication should be strong, all data should be encrypted, and because all of that can still fail, all traffic should be logged and monitored for aberrance to mitigate damage and facilitate post-mortems. 
\cite{the actual zero trust model thingy from palo alto} 

While some of these principles have been extended to consumer technology, such as the omnipresence of strong encryption, not all have, nor is it necessarily pragmatic or desirable to do so. 
For myriad reasons, people cannot, do not wish to, and will not strictly limit access to their network of devices and accounts. People have financial, cultural, and interpersonal constraints which prevent them from keeping devices and users 1:1. People wish to extend an infosec understanding of trust to those with whom they share \textit{human trust.}
Users do not enjoy, nor prefer to use, complicated strong authentication schemes. When it is avoidable, most avoid it. \cite{} 

Consumer technology engages in constant logging and monitoring - as a zero trust corporate network would - though this is not done in a manner that is visible to the consumer, nor is it done strictly for their benefit. In cases where users have issues within their "network" this logging can provide useful information: Find My iPhone can be used to locate a lost or stolen device, and [another example.] Google logs and analyzes everything because they have a material interest in doing so. As a byproduct, they are able to provide individuals with alerts to suspicious activity within their accounts. \cite{I'm sure google has something on this} 

Work has been done to 'nudge' consumers towards better security practices \cite{} and to create new methods of authentication and make them more usable \cite{}. These are steps towards better security and privacy for consumers, but still ignore the fundamental tension: consumers are human, and they wish to act like it. Humans do not live in a world where zero trust is a gold standard -- quite the opposite. 

This work focuses on illustrating the ways in which people share access to their "network" with those they trust most: their romantic partners. Through a large-scale survey, we provide empirical data and discuss peoples' behavior in practice with respect to their phones and their partners, as well as perceptions of cultural and moral norms. 
We illustrate that there is little consensus among demographic groups about what behavior is desirable or acceptable, and often there is not consensus within groups. 
Through the usage of free-text responses we show that consumers understand nuance in these contexts, noting where certain behaviors could be both good or bad, depending upon the circumstances. Users draw heavily on the idea of \textit{trust} within a relationship to explain why something is good; sometimes, this is complete privacy from a spouse, for others it's complete transparency. 
There does not seem to be a consensus on what an appropriate level of access to a partner's network of devices and accounts is, only that such access should be consensual and that limits must be respected. While healthy communication and trust are obviously important in romantic relationships, these delineations must be drawn so firmly because it is essentially impossible to give a partner access to only that which one deems it appropriate to give access to. In giving one's partner their phone PIN, one bequeaths access to all of their accounts, their two factor token, and the email that resets all of their passwords - i.e. their entire "network." 

In assuming a single point of access control, we rely very heavily on users not doing the very human thing of sharing, or we rely heavily on \textit{human trust}, which is certainly fallible. In cases of intimate relationships, all manner of breeches of trust can occur, and because the access is there, the consequences can be severe. One's partner may access messages without permission, monitor search or location history, or even go so far as to install spyware on their device. As these behaviors move on the sliding scale towards abuse, there is little to be done to remediate them, because it is incredibly difficult to remove access someone already has, particularly in a violent context. 

While a true Zero Trust Model is also intractible in interpersonal contexts, a reevaluation of the design assumptions that favor a trend towards strong authentication as a modus of consumer protections rather than a shift to more granular access control might go a long way.

Designing systems to be as human-proof as possible may be viable in a corporate context where everyone can be required to use a hardware token and take phishing prevention trainings, downloads and website access can be restricted, and policies can be enforced on the threat of losing one's livelihood. Consumers, on the other hand, cannot and should not have such limitations imposed upon them with devices and accounts that they pay for (either in money or in data), so it is pertinent to consider new ways of designing security models that align with how people actually behave. 

old sharing

A large majority of individuals in romantic relationships give their partners access to their smartphones, and receive access in return. Because one's phone is the lynch pin in one's network of devices and accounts, this act endows a great deal of trust, which is not always respected. 

We asked respondents who had access to their partner's phone about how they made use of that access. We asked about both benign, banal behaviors and invasive behaviors, in the hope of establishing a baseline.
The data from Symantec asked some similar questions relating to snooping behaviors. In places where the two datasets overlap, the proportions of respondents acknowledging a behavior are quite similar. 

\subsection{Passive v. Active behaviors}

\peri{this carries into attitudes and I'm not sure whether to keep it here or how to split so just gonna keep going for now - this section is obviously not done but idk what else to put here so maybe we should just condense with the next one}

With respect to actual behavior, as well as perceptions of whether behavior was good or common, there were gendered differences. Women were more ready to accept and condone snooping behaviors that were passive, like reading a partner's texts, while men were more willing to take active measures, like calling a number from their partner's call history.

==> privacy.tex <==
\subsection{"I don't need to know, I trust him."}




==> secposture.tex <==
\section{Security Posture}
Despite the fact that one's smartphone is essentially the singular key to one's digital ecosystem, people do not engage in strong security practices with them. 

\peri{add some info perhaps about Android/Google and iOS/iCloud and how they work and how they oAuth etc. and auth types so on so forth}

\subsection{Access Control}
We asked respondents, regardless of their relationship status, about their phone's security posture. We asked whether it locked, and then which types of locks they used.

\peri{this obviously should get tables but before I put in the effort thought I'd get feedback on what's useful to avoid the data dump}
\begin{itemize}
    \item 86\% of respondents said their phone locks when they turn it off
    \item Men were significantly more likely than women to have a lock on their phone (90 v 82)
    \item iPhone users were significantly more likely to have a lock on their phone than Android users (92 v 81) - I mention this because it is perhaps an illustration that defaults and design choices can inform security practices, though it may also be a byproduct of demography. 
    \item Individuals in very serious relationships (married, engaged, civil union, domestic partnership) were the least likely to have a lock on their phone (81), while those who were in relationships that were less serious were the most likely (89). This difference is significant. (of course, there is the relation with age here too, younger people are more likely to have a locked phone than older people, and older people are more likely to have serious relationships, the directionality of this isn't clear)
    \item those who said they were not or somewhat familiar with technology were significantly less likely to have a lock on their phone that those who said they were quite familiar or experts. (81 v 89)
    \item of users whose phones locked, 69\% reported using a biometric lock, either facial recognition or fingerprint
    \item between types of authentication, there are demographic differences, but these are attributable to OS choice (e.g. young people much more likely to have 6 digit PIN because they were more likely to use iOS)
    \item 10\% of respondents who reported that their phone locked indicated that they use an alphanumeric password to lock their phone
\end{itemize}

\subsection{Access Within Relationships}
For respondents who indicated they were in a romantic relationship, we asked about their partner's access to their phone. If they indicated that their phone did not lock, we assumed that their partner had access to it, unless they had indicated they were in a long distance relationship. For each type of lock the respondent indicated they had enabled, we asked whether their partner had access, for example, if they indicated they use a PIN, does their partner know that PIN? If they indicated they used facial recognition, is their partner able to unlock their phone with their own face?

Key takeaways: most people do give their partner access, but are much less likely to give biometric access than PIN.

\begin{itemize}
    \item 67\% of respondents in relationships indicated that their partner had access to their phone, including 14\% whose phone did not lock and 52\% whose partner had explicit access.
    \item Those in very serious relationships were significantly more likely to have a partner with access than those in less serious relationships (75 v. 58)
    \item Women were significantly more likely than men to have a partner with access than men (73 v. 58) there are not significant age or relationship statuses amongst men and women in the sample
    \item Of users in relationships who unlocked their phone biometrically, 17\% reported that their partner had independent biometric access to their device, while 44\% reported that their partner had access to their device, but not biometric access.
    \item Neither mobile OS allows for biometric access as the only uathentication mechanism, with iOS requiring a PIN or password, and Android allowing a swipe pattern as well. Of users in relationships whose device locked using a PIN or swipe pattern (all, except those using passwords), 66\% reported that their partner knew the PIN or swipe pattern to unlock their device. 
    \item Of users who reported that their partner had access to their device, 98\% indicated that their partner knew their PIN or swipe pattern, with only 2 respondents indicating their partner had biometric access but didn't know their PIN. 
    \item 3 respondents who used a password in place of a PIN indicated that their partner had fingerprint access, but not their password. One wonders if this is a workaround for corporate BYOD requirements, but we have no indication on this front. 
\end{itemize}

We also asked respondents in relationships about their partner's phone, whether it locked, how it locked, and if they were able to independently unlock it. 

\peri{add this data}

\subsection{Symmetry of access}

For respondents with partners, we were able to ascertain whether they had access to their partners' device, whether their partner had access to theirs, and whether their was parity. For the most part, there was. The vast majority of respondents reported that they either both had access to each others' devices, or both did not. 
\begin{itemize}
    \item Women were significantly more likely to report that they and their partner had mutual access (63 v 46), while men were more likely to report that they and their partner had mutual non-access (30 v 19). \item there were not significant gender differences across states of asymmetry, nor a propensity to exist in a state of asymmetry
    \item Given that the vast majority of relationships are heterosexual , it is not possible for 63\% of women to be in relationships with mutual access while only 46\% of men are in relationships with mutual access. 
    \item It is possible that there is a bias in the sample which impacts this, though the crosstabs don't reflect any major ways in which men and women in our sample differ. women are less likely to have a phone which locks, which implies access, but this does not negate the point above. 
    \item there are well established differences between the way men and women in the same relationship report behavior, so it is also possible that this is a semblance of what is correct, and two populations are counting differently.
    \item Those is 'serious' relationships were significantly more likely to report that they had mutual access, while those in less serious relationships reported mutual non-access. 
    \item comparisons across age and sexual orientation were not significant
    
\end{itemize}


==> survey_format.tex <==
What Platform were you referred from?
\begin{itemize}
    \item Prolific
    \item Facebook Ad
\end{itemize}

What country do you live in?

How old are you?

Do you use a smartphone on a daily basis?

You indicated you were referred from Prolific, please provide your ID. We will not retain this information after your survey is approved and your reward distributed.

What is your gender identity?
\begin{itemize}
    \item Female
    \item Male
    \item Non-Binary
    \item Other
\end{itemize}

What is your current marital status?
\begin{itemize}
    \item Never Married
    \item Divorced
    \item Widowed
    \item Currently Married
    \item Engaged
    \item Married, but separated
    \item Common Law Marriage, Domestic Partnership, or Civil Union
\end{itemize}
 
Which of these apply to you right now?
\begin{itemize}
    \item I have a sexual or intimate relationship with someone
    \item I am in a serious relationship
    \item I am dating or going out with someone
    \item I am in another type of close romantic relationship
    \item None of these apply to me right now
\end{itemize}

Do you and your partner live together?
\begin{itemize}
    \item Yes
    \item No
\end{itemize}

Are you and your partner in a long distance relationship?
\begin{itemize}
    \item Yes
    \item No
\end{itemize}

What is the gender identity of your partner?
\begin{itemize}
    \item Female
    \item Male
    \item Non-Binary
    \item Other
\end{itemize}

Tech Questions – all participants

What kind of smartphone do you have?
\begin{itemize}
    \item Android
    \item iPhone
    \item Other
\end{itemize}

How would you describe your level of familiarity with technology?
\begin{itemize}
    \item I use my phone for texting and calls, and simple apps like directions, weather, and music
    \item iPhone
    \item Other
\end{itemize}

•	
o	Android (such as Samsung, Pixel, LG, Motorola, Huawei, etc.)
o	iPhone
o	Other please specify
•	
o	I use it for texting and calls, and simple apps like directions, weather, and music
o	I use many apps for many different things
o	I  use many apps and I know a lot about my phone’s features and settings
o	I am a super user/I work in technology or am a developer
•	If you own or use more than one smartphone, please consider your primary personal smartphone going forward.
•	Regardless of who pays for it, are you and your partner on the same cell plan?
o	No
o	Yes

Security Status Quo – all participants

•	Does your phone lock when you turn it off?
o	Yes
o	No
•	[if yes above] How does your phone lock? Select all that apply
1.	4 digit PIN
2.	6 digit PIN
3.	Swipe pattern
4.	Fingerprint recognition
5.	Facial Recognition
•	You indicated your phone can be unlocked with a PIN, does your partner know the PIN that unlocks your phone?
o	Yes
o	No
o	I don’t know
•	You indicated your phone can be unlocked with a swipe pattern, does your partner know the swipe pattern that unlocks your phone?
o	Yes
o	No
o	I don’t know
•	You indicated that your phone can be unlocked using a fingerprint, is your partner able to unlock your phone using THEIR OWN FINGERPRINT?
o	Yes
o	No
•	You indicated that your phone can be unlocked using facial recognition, is your partner able to unlock your phone using THEIR OWN FACE?
o	Yes
o	No

Tech Questions – partner, if applicable
•	Which does your partner use for their primary phone?
1.	Android (such as Samsung, Pixel, LG, Motorola, Huawei, etc.)
2.	iPhone
3.	Cell phone which is not a smart phone, such as flip phone or trac phone
4.	Landline
5.	My partner does not use a phone
•	Questions about partner’s phone will be asked if answer above is 1 or 2
•	How would you describe your partner’s level of familiarity with their phone?
1.	They use it for texting and calls, and simple apps like directions, weather, and music
2.	They use many apps for many different things
3.	They  use many apps and I know a lot about my phone’s features and settings
4.	They are a super user/I work in technology or are a developer
•	Does your partner’s phone lock when they turn it off?
o	Yes
o	No
•	[if yes above] How does their phone lock? Select all that apply
1.	4 digit PIN
2.	6 digit PIN
3.	Swipe pattern
4.	Fingerprint recognition
5.	Facial Recognition
6.	I don’t know how their phone locks
The following questions are asked as applicable
•	You indicated your partner’s phone can be unlocked with a PIN, do you know the PIN that unlocks your partner’s phone?
o	Yes
o	No
•	You indicated your partner’s phone can be unlocked with a swipe pattern, do you know the swipe pattern that unlocks your partner’s phone?
o	Yes
o	No
•	You indicated that your partner’s phone can be unlocked using a fingerprint, are you able to unlock your partner’s phone using YOUR OWN FINGERPRINT?
o	Yes
o	No
•	You indicated that your partners’ phone can be unlocked using facial recognition, are you able to unlock your partner’s phone using YOUR OWN FACE?
o	Yes
o	No



Questions about use of access – only if in relationship AND has access to partner phone

These questions ask about a list of behaviors, along the scale below

•	You indicated that you have access to your partner’s phone. For each of the following behaviors, indicate how often you would do this.
o	Never
o	Seldom
o	Sometimes, if my partner asks me to
o	Sometimes, if my partner is not in the room
o	Often
•	Behaviors – first page
o	Change the music
o	Get directions
o	Look something up, like a recipe or how old a celebrity is
o	Look at their saved places or location history
•	Behaviors – second page
o	Look at their search history
o	Look at their call history
o	Make a phone call
o	Send a text
o	Look at who my partner has been texting
o	Read the contents of my partners text conversations
•	Behaviors – third page
o	Open my partner’s social media apps
o	Look at my own profile from my partner’s social media account
o	Look through my partner’s social media account activity
o	Read my partner’s direct messages from within their social media account
o	Take action from my partner’s social media account, such as deleting friends or posting, editing a post, etc.
•	Behaviors – fourth page
o	Look at the list of apps they have installed
o	Install an app that tracks them, or relays information back to me 
o	Open my partner’s phone to help them with a tech issue


Societal perceptions – all participants

These questions ask about the same behaviors, in a list, with the scales below for each behavior. 

•	For each of the behaviors listed, please indicate how COMMON you think it is for people in relationships to do this behavior
1.	Very uncommon
2.	Somewhat uncommon
3.	Somewhat common
4.	Very common
5.	I don’t know what this is
•	For each of the behaviors listed, please indicate whether you think the behavior is GOOD or HEALTHY in the context of a relationship, or BAD or TOXIC in the context of a relationship
1.	This behavior is GOOD or HEALTHY
2.	This behavior is NORMAL but could be problematic
3.	This behavior is PROBLEMATIC but could be justified
4.	This behavior is BAD or TOXIC
5.	I don’t know what this is
•	Behaviors – first page
1.	Sharing a phone PIN or swipe pattern
2.	Giving partner ability to unlock phone with their own fingerprint of faceID
3.	Sharing a password to social media accounts
4.	Sharing an email password
5.	Sharing a password to streaming accounts
•	Behaviors – second page
1.	Sharing location on an ongoing basis
2.	Sharing an online storage account
3.	Using a couple’s tracking app
4.	Installing a hidden tracking app
5.	Sharing a bank account
6.	Sharing a phone plan
•	Behaviors – third page
1.	Looking at partner’s search history
2.	Looking at partner’s location history
3.	Looking through partner’s call history on their phone
4.	Looking at partner’s call history on the phone bill
5.	Looking through partner’s text history
•	Behaviors – fourth page
1.	Looking at partner’s social media activity from your own account
2.	Logging into partner’s social media account
3.	Logging into partner’s social media account and reading direct messages
4.	Logging into partner’s social media account and taking an action
5.	Confronting partner about something they did on social media

Abuse Screener – only for those in relationships

•	Now we’re going to ask some questions about behavior in relationships that are negative or harmful, which could be upsetting. if you don’t want to answer these questions, you can skip them.
1.	I’m ok answering them
2.	I am uncomfortable answering them
•	Questions below all have the same scale:
1.	Never
2.	Once
3.	A few times
4.	Regularly
•	In the entire time you’ve been together, how often has your partner done the following?
1.	Kept you from using your phone to communicate with others
2.	Kept you from using your phone for some other reason
3.	Changed your passwords without your consent
4.	Damaged or broken your phone
•	In the entire time you’ve been together, how often has your partner done the following?
1.	Used or accessed your phone while pretending to be you
2.	Accessed your phone to look at your text, email, or social media accounts without your consent
3.	Accessed your phone to check your location or activities without your consent
4.	Accessed your phone to install spyware on it
•	In the entire time you’ve been together, how often has your partner done the following?
1.	Become jealous or possessive
2.	Tried to provoke arguments
3.	Called you derogatory names
4.	Purposely tried to make you feel inadequate
•	In the entire time you’ve been together, how often has your partner done the following?
1.	Threatened to harm you
2.	Threatened to harm someone else
3.	Threatened to harm themselves
•	In the entire time you’ve been together, how often has your partner done the following?
1.	Become physically aggressive with you
2.	Made you do something sexual you really didn’t want to
•	In the entire time you’ve been together, how often have you done the following to avoid angering or ‘setting off’ your partner?
1.	Avoided spending time with friends or family
2.	Avoided spending money on something you needed
3.	Given access to my phone
4.	Stopped driving
5.	Quit a job you didn’t want to quit
6.	Changed educational plans you didn’t want to change

Demographic questions
•	Which of these represent your racial or ethnic identity? Select all that apply
1.	African descent (Black, African-American)
2.	East Asian
3.	European descent (White, Caucasian)
4.	Hispanic or Latino
5.	Middle-Eastern descent
6.	Native American, or other Native People
7.	Pacific Islander
8.	South Asian
•	Regardless of your citizenship status, do you consider the US your home?
1.	Yes
2.	No
•	[if yes above] Which best applies to you?
1.	I have lived in the US my entire life
2.	I immigrated to the US
3.	I was born in the US, but have lived a significant portion of my life abroad
•	[if immigrated] At what age did you immigrate?
1.	Before school [0-5]
2.	Grade school [6-12]
3.	Secondary school [13-17]
4.	Young adult [18-29]
5.	Adult [30+]
•	[if US entire life] Which of these apply to your family? Select all that apply
1.	One of my parents immigrated to the US
2.	Both of my parents immigrated to the US
3.	One or more of my grandparents immigrated to the US
4.	My family speaks a language other than English at home, or in addition to English
•	What is the highest level of education you have completed?
1.	Have not finished high school
2.	High school
3.	Associates degree, professional licensure or certification
4.	Bachelor’s degree
5.	Graduate or professional degree
•	Which of the following best describes your financial situation?
1.	I struggle to pay bills and put food on the table
2.	I make ends meet, but that’s about it. I have short-term debt like credit card debt.
3.	I have everything I need, I’m saving a little for the future, and I can afford a few nice things. I have long term debt like student loans or a mortgage.
4.	I have everything I need, I have no debt, I have most things I want
•	Which of the following best describes your partner’s financial situation?

Demographic questions about partner, if applicable
•	How old is your partner?
•	What is the highest level of education your partner has completed?
o	Same options as question about participant’s education
•	Which best describes your financial situation with respect to your partner?
1.	We do not have shared expenses or accounts
2.	We have shared expenses but not shared accounts
3.	We have shared expenses and shared accounts
•	[is answer to above is 1 or 2] Which best describes your partner’s financial situation?
1.	They are worse off than me financially
2.	We are in about the same situation financially
3.	They are better off than me financially
4.	I don’t know what my partner’s financial situation is

Abuse and cyber security resources

Finalization

If from MTurk, completion code

If from Prolific, completion code

If from other platform, drawing entry code



==> table_access_type.tex <==
\begin{table}[]
\begin{tabular}{lll|l|ll|l}
                                                                        & PIN   & Swipe & SYK   & Fingerprint & \begin{tabular}[c]{@{}l@{}}Facial\\ Recognition\end{tabular} & Biometric \\ \hline
\begin{tabular}[c]{@{}l@{}}Respondents\\ Using\end{tabular}             & 154   & 48    & 189   & 96          & 66                                                           & 139       \\
\begin{tabular}[c]{@{}l@{}}\% Partners\\ with Access\end{tabular}       & 0.974 & 0.896 & 0.952 & 0.323**     & 0.136**                                                      & .273      \\ \hline
\begin{tabular}[c]{@{}l@{}}Partners\\ Using\end{tabular}                & 137   & 28    & 162   & 53          & 56                                                           & 99        \\
\begin{tabular}[c]{@{}l@{}}\% Respondents\\ \\ with Access\end{tabular} & 0.985 & 0.786 & 0.957 & 0.434**     & 0.214**                                                      & 0.343    
\end{tabular}

\caption{Access type, among those whose partners have access}
~\label{tab:access_type}
\end{table}

==> table_auth_os.tex <==
\begin{table}[]
    \begin{threeparttable}

\begin{tabular}{l|ll|lll|l}
        & N   & \begin{tabular}[c]{@{}l@{}}Phone\\ Locks\end{tabular} & N   & \begin{tabular}[c]{@{}l@{}}Facial\\ Recognition\end{tabular} & \begin{tabular}[c]{@{}l@{}}Fingerprint\\ Sensor\end{tabular} & \begin{tabular}[c]{@{}l@{}}Either\\ Biometric\end{tabular} \\ \hline
Total   & 552 & 0.837                                                 & 389 & 0.285                                                        & 0.463                                                        & 0.679                                                      \\ \hline
Android & 253 & 0.81\tnote{*}                                                 & 204 & 0.157                                                        & 0.539                                                        & 0.564\tnote{**}                                                    \\
iOS     & 206 & 0.922\tnote{*}                                                & 184 & 0.429                                                        & 0.38                                                         & 0.81\tnote{**}                                                    
\end{tabular}

\begin{tablenotes}

\small\item[*] Significant difference in frequency of locking, p-value = 0.004

\item[**] Significant difference in frequency of biometric use, p-value < 0.0001
\end{tablenotes}
    \end{threeparttable}

\caption{Authentication types enabled by operating system}

~\label{tab:auth_os}
\end{table}

==> table_rel_stat_lock.tex <==
\begin{table}[]
\begin{tabular}{l|ll|ll|ll}
             & \multicolumn{2}{l}{Respondents}                             & \multicolumn{2}{|l}{Partners}                                & \multicolumn{2}{|l}{Total}                                   \\ 
             & N   & \begin{tabular}[c]{@{}l@{}}\% Locks\end{tabular} & N   & \begin{tabular}[c]{@{}l@{}}\% Locks\end{tabular} & N   & \begin{tabular}[c]{@{}l@{}}\% Locks\end{tabular} \\ \hline
All          & 552 & .837                                                  & 341 & .78                                                   & 893 & .815                                                  \\ \hline
Single       & 143 & .797                                                  & NA  & NA                                                    & 143 & .797                                                  \\ \hline
Has Partner  & 409 & .851                                                  & 341 & .78                                                   & 750 & .819                                                  \\ \hline
Serious      & 210 & .8                                                    & 178 & .753                                                  & 388 & .778                                                  \\ \hline
Less Serious & 199 & .904                                                  & 163 & .81                                                   & 362 & .862                                                  \\
\end{tabular}
\caption{Fraction of individuals whose phones lock by relationship status}
~\label{tab:rel_stat_lock}
\end{table}
